Secure Cloud Assisted Smart Cars Using Dynamic Groups and Attribute Based Access Control

Future smart cities and intelligent world will have connected vehicles and smart cars as its indispensable and most essential components. The communication and interaction among such connected entities in this vehicular internet of things (IoT) domain, which also involves smart traffic infrastructure, road-side sensors, restaurant with beacons, autonomous emergency vehicles, etc., offer innumerable real-time user applications and provide safer and pleasant driving experience to consumers. Having more than 100 million lines of code and hundreds of sensors, these connected vehicles (CVs) expose a large attack surface, which can be remotely compromised and exploited by malicious attackers. Security and privacy are serious concerns that impede the adoption of smart connected cars, which if not properly addressed will have grave implications with risk to human life and limb. In this research, we present a formalized dynamic groups and attribute-based access control (ABAC) model (referred as \cvac) for smart cars ecosystem, where the proposed model not only considers system wide attributes-based security policies but also takes into account the individual user privacy preferences for allowing or denying service notifications, alerts and operations to on-board resources. Further, we introduce a novel notion of groups in vehicular IoT, which are dynamically assigned to moving entities like connected cars, based on their current GPS coordinates, speed or other attributes, to ensure relevance of location and time sensitive notification services to the consumers, to provide administrative benefits to manage large numbers of smart entities, and to enable attributes and alerts inheritance for fine-grained security authorization policies. We present proof of concept implementation of our model in AWS cloud platform demonstrating real-world uses cases along with performance metrics.

==> Figures/lg1.tex <==
%\newpage
\begin{figure}[t]
\centering
\includegraphics[scale=.45]{Figures/lg1-v7}
\caption{Representative Groups Hierarchy}
\label{fig gh}
\end{figure}


==> Figures/numbers.tex <==
\begin{figure}[t]
\centering
\includegraphics[scale=.75]{Figures/numbers-v3}
\caption{Policy Enforcement Time and Scoping}
\label{fig-num}
\end{figure} 



==> Sections/Implementation.tex <==
\section{Implementation in AWS}



==> Sections/Performance.tex <==
\section{Performance Evaluation} \label{eval}

==> Tables/table_model.tex <==
\begin{table*}\label{tab1}
\centering
%\captionsetup{justification=centering}
\caption{Formal \cvac~Model Definitions for Connected Vehicles Ecosystem}% \\ (\textsuperscript{**} and \textsuperscript{++} highlights new and modified components respectively w.r.t \heac)}
\label{tab 1}
%\resizebox{\textwidth}{!}
%\resizebox*{!}{\totalheight}
{%
\begin{tabular}{@{}llllll@{}}
\toprule
\multicolumn{6}{l}{\textbf{Basic Sets and  Functions}}\\
\multicolumn{6}{l}{-- S, CO, O, G, OP are finite sets of sources, clustered objects, objects, groups and operations respectively [blue circles in Figure \ref{fig model}].}                              \\
%\multicolumn{6}{l}{-- HS, \ophs (finite set of Hadoop services and operations respectively)}                                                      \\
%\multicolumn{6}{l}{-- HS, ES are finite sets of Hadoop services and ecosystem services respectively.}                                                      \\
%\multicolumn{6}{l}{-- G, OP are finite sets of groups and operations respectively.}                                                      \\
\multicolumn{6}{l}{-- A is a finite set of activities which can be performed in system.}                                                      \\
\multicolumn{6}{l}{-- ATT is a finite set of attributes associated with S, CO, O, G and system-wide.}                                                      \\
\multicolumn{6}{l}{-- For each attribute att in ATT,  Range(att) is a finite set of atomic values.}
\\
\multicolumn{6}{l}{-- attType: ATT = \{set, atomic\}, defines attributes to be set or atomic valued.}                                                      \\
\multicolumn{6}{l}{\begin{tabular}{@{}l@{}}-- Each attribute att in ATT maps entities in S, CO, O, G to attribute values. Formally,\\\;\; att : S $\cup$ CO $\cup$ O $\cup$ G $\cup$ \{system-wide\} $\rightarrow$\; $ \begin{cases} \mathrm{{Range(att)}}~\cup \{\bot\} & \text{if attType(att) = atomic}\\ \mathrm{2^{Range(att)}} & \text{if attType(att) = set} \\ \end{cases}$ \end{tabular}}
\\
\multicolumn{6}{l}{-- POL is a finite set of authorization policies associated with individual S, CO, O, G.}                                                      \\
\multicolumn{6}{l}{-- directG : $ \mathrm{CO \rightarrow {G}} $,  mapping each clustered object to a system group, equivalently CGA $ \subseteq \mathrm{CO} \times \mathrm{G}. $}
%\multicolumn{6}{l}{-- directG : $ \mathrm{CO \rightarrow 2^{G}} $,  mapping each clustered objects to a set of groups, equivalently CGA $ \subseteq \mathrm{CO} \times \mathrm{G}. $}
\\
\multicolumn{6}{l}{-- parentCO : $ \mathrm{O \rightarrow CO} $,  mapping each object to a clustered object, equivalently OCA $ \subseteq \mathrm{O} \times \mathrm{CO}. $}
\\
%\multicolumn{6}{l}{-- rootparentG : $ \mathrm{G \rightarrow G} $,  mapping each group to root parent group in hierarchy.}
%\\
\multicolumn{6}{l}{-- $\mathrm{GH \subseteq G~\times}$ G,  a partial order relation $\succeq_{\textit{g}}$ on G. Equivalently, parentG : $\mathrm{G \rightarrow 2^{G}}$, mapping group to a set of parent groups in hierarchy.}                                                                                                          \\
%\multicolumn{6}{l}{-- parentG : $ \mathrm{G \rightarrow 2^{G}} $,  mapping each group to set of parent groups in hierarchy, equivalently GH $\subseteq$ G $\times$ G.}
%\multicolumn{6}{l}{-- rootGroup : $ \mathrm{G \rightarrow G} $,  mapping each group to root parent group in hierarchy.}
\\
\multicolumn{1}{l}{\textbf{Effective Attributes of Groups, Clustered Objects and Objects (Derived Functions)}}                                                                 \\
%\multicolumn{6}{l}{\begin{tabular}{@{}l@{}}-- Each attribute att in ATT maps entities in S, CO, O, G to attribute values. Formally,\\\;\; $\mathrm{\effg_{att}}$ : G $\rightarrow$\; $ \begin{cases} \mathrm{{Range(att)}} & \text{if attType(att) = atomic, defined as $\mathrm{\effg_{att}(g_i)}$ = $\mathrm{att(g_i)}$ $\cup$  $\mathrm{\effg_{att}(g_j)}$ such that $\mathrm{{ g_i \; \succeq_{\textit{g}}\; g_j }}$}\\ \mathrm{2^{Range(att)}} & \text{if attType(att) = set} \\ \end{cases}$ \end{tabular}}\\
%\multicolumn{6}{l}{\begin{tabular}[c]{@{}l@{}}-- For each attribute $\mathrm{att}$ in ATT such that attType(att) = set: \\ $ \;\;\;\; \bullet \;\;$ $\mathrm{\effg_{att}}$ : \Gr~$\rightarrow {2^{\range}}$, defined as $\mathrm{\effg_{att}(g_i)}$ = $\mathrm{att(g_i)}$ $\cup$  $ (\mathrm{\bigcup\limits_{ g \; \in\; \{g_j | g_i \; \succeq_{\textit{g}}\; g_j\} } \effg_{att}(g))}$. \end{tabular}} \\
\multicolumn{6}{l}{\begin{tabular}[c]{@{}l@{}}-- For each attribute $\mathrm{att}$ in ATT such that attType(att) = set: \\ $ \;\;\;\; \bullet \;\;$ $\mathrm{\effg_{att}}$ : \Gr~$\rightarrow {2^{\range}}$, defined as $\mathrm{\effg_{att}(g_i)}$ = $\mathrm{att(g_i)}$ $\cup$  $ (\mathrm{\bigcup\limits_{ g \; \in\; \{g_j | g_i \; \succeq_{\textit{g}}\; g_j\} } \effg_{att}(g))}$. \end{tabular}} \\
%\multicolumn{6}{l}{\begin{tabular}[c]{@{}l@{}}-- For each attribute $\mathrm{att}$ in ATT such that attType(att) = set: \\ $ \;\;\;\; \bullet \;\;$ $\mathrm{\effg_{att}}$ : \Gr~$\rightarrow {2^{\range}}$, defined as $\mathrm{\effg_{att}(g_i)}$ = $\mathrm{att(g_i)}$ $\cup$  $\mathrm{\effg_{att}(g_j)}$ such that $\mathrm{{ g_i \; \succeq_{\textit{g}}\; g_j }}$. \end{tabular}} \\
\multicolumn{6}{l}{\begin{tabular}[c]{@{}l@{}}$ \;\;\;\; \bullet \;\;$ $\mathrm{\effu_{att}}$ : CO~$\rightarrow {2^{\range}}$, defined as $\mathrm{\effu_{att}(co)}$ = $\mathrm{att(co)}$ $\cup$  $ \mathrm{ \effg_{att}(directG(co))}$. \end{tabular}} \\
\multicolumn{6}{l}{\begin{tabular}[c]{@{}l@{}}$ \;\;\;\; \bullet \;\;$ $\mathrm{\effo_{att}}$ : O~$\rightarrow {2^{\range}}$, defined as $\mathrm{\effo_{att}(o)}$ = $\mathrm{att(o)}$ $\cup$  $\mathrm{ \effu_{att}(parentCO(o))}$. \end{tabular}} \\
%\multicolumn{6}{l}{\begin{tabular}[c]{@{}l@{}}-- For each attribute $\mathrm{att}$ in ATT such that attType(att) = atomic: \\ $ \;\;\;\; \bullet \;\;$ $\mathrm{\effg_{att}}$ : \Gr~$\rightarrow {{\range}}$, defined as $\mathrm{\effg_{att}(g_i)}$ = $\mathrm{\effg_{att}(g_j)}$ such that $\mathrm{{ g_i \; \succeq_{\textit{g}}\; g_j }}$. \end{tabular}} \\
\multicolumn{6}{l}{\begin{tabular}[c]{@{}l@{}}-- For each attribute $\mathrm{att}$ in ATT such that attType(att) = atomic: \\ $ \;\;\;\; \bullet \;\;$ $\mathrm{\effg_{att}}$ : \Gr~$\rightarrow {{\range}} \cup \{\bot\}$, defined as $\mathrm{\effg_{att}(g_i)}$ = $ \begin{cases} \mathrm{att(g_i)} & \text{if $\forall \mathrm{g'} \in \mathrm{parentG(g_i)}.~ \mathrm{\effg_{att}(g')} = \bot$}\\ \mathrm{\effg_{att}(g')} & \text{if $\exists~\mathrm{parentG(g_i)}.~ \mathrm{\effg_{att}(parentG(g_i))} \neq \bot$ then select}\\ & \text{parent $\mathrm{g'}$ with $\mathrm{\effg_{att}(g')} \neq \bot$ updated most recently.}\end{cases}$ \end{tabular}} \\
\multicolumn{6}{l}{\begin{tabular}[c]{@{}l@{}}$ \;\;\;\; \bullet \;\;$ $\mathrm{\effu_{att}}$ : CO~$\rightarrow {{\range}} \cup \{\bot\}$, defined as $\mathrm{\effu_{att}(co)}$ = $ \begin{cases} \mathrm{att(co)} & \text{if $\mathrm{\effg_{att}(directG(co))} = \bot$}\\ \mathrm{\effg_{att}(directG(co))} & \text{otherwise}\\ \end{cases}$ \end{tabular}} \\
\multicolumn{6}{l}{\begin{tabular}[c]{@{}l@{}}$ \;\;\;\; \bullet \;\;$ $\mathrm{\effo_{att}}$ : O~$\rightarrow {{\range}} \cup \{\bot\}$, defined as $\mathrm{\effo_{att}(o)}$ = $ \begin{cases} \mathrm{att(o)} & \text{if $\mathrm{\effu_{att}(parentCO(o))} = \bot$}\\ \mathrm{\effu_{att}(parentCO(o))} & \text{otherwise}\\ \end{cases}$ \end{tabular}} \\
\midrule
\multicolumn{2}{l}{ \textbf{Authorization Functions (Policies)}}                                                                                                          \\
\multicolumn{6}{l}{\begin{tabular}[c]{@{}l@{}}-- {Authorization Function:} For each op $\in$ OP, $\mathrm{Auth_{op}(s:S, ob:CO \cup O \cup G)}$ is a propositional logic formula  returning true or false, \\\;\; which is defined  using the following policy language: \end{tabular}}\\
\multicolumn{6}{l}{\begin{tabular}[c]{@{}l@{}}$\;\;\;\; \bullet \;\; \mathrm{ \alpha \Coloneqq \alpha \land \alpha \;|\; \alpha \vee \alpha \;|\; (\alpha) \;|\; \neg \alpha \;|\; \exists\; x \in set.\alpha  \;|\; \forall\; x \in set.\alpha \;|\;  set \bigtriangleup set \;|\; } $ $ \mathrm{atomic \in set \;|\;  atomic \notin set }$\end{tabular}} \\

\multicolumn{6}{l}{$ \;\;\;\; \bullet \;\; \bigtriangleup \Coloneqq  \; \subset \;|\; \subseteq \;|\; \nsubseteq \;|\; \cap \;|\; \cup $}\\
\multicolumn{6}{l}{$ \;\;\;\; \bullet \;\;\mathrm{  set \Coloneqq {eff}_{att}(i) \;|\; {att}(i) }$}for $\mathrm{att}$ $\in $ ATT, i $\in$ S $\cup$ CO $\cup$ O $\cup$ G $\cup$ \{system-wide\}, attType(att) = set \;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\\
\multicolumn{6}{l}{$ \;\;\;\; \bullet \;\; \mathrm{ atomic \Coloneqq {eff}_{att}(i) \;|\; {att}(i) \;|\; value }$} for $\mathrm{att}$ $\in $ ATT, i $\in$ S $\cup$ CO $\cup$ O $\cup$ G $\cup$ \{system-wide\}, attType(att) = atomic \;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\\
\midrule
\multicolumn{2}{l}{ \textbf{Authorization Decision}}                                                                                                          \\
\multicolumn{6}{l}{\begin{tabular}[c]{@{}l@{}}-- A source $\mathrm{s}$ $\in$ S is allowed to perform an activity a $\in$ A, stated as $\mathrm{Authorization(a:A, s:S)}$, if the required policies needed to allow \\\;\; the activity are included and evaluated to make final decision. These multi-layer policies must be evaluated for individual \\\;\; operations ($\mathrm{op_i}$ $\in$ OP) to be performed by source s $\in$ S on relevant objects ($\mathrm{x_i}$ $\in$ CO $\cup$ O $\cup$ G). \\\;\; Formally,
$\mathrm{Authorization(a:A, s:S)}$ $\Rightarrow$ $\mathrm{Auth_{op_1}(s:S, x_1)}$, $\mathrm{Auth_{op_2}(s:S, x_2)}$, $\ldots$ $\ldots$ $\ldots$ $\ldots$, $\mathrm{Auth_{op_n}(s:S, x_3)}$
%$\mathrm{Authorization_{a}(s:S, ob:CO \cup O \cup G)}$.\\\;\; Formally, $\mathrm{Authorization_{access}(s:S, es:ES)}$ = True $\land$ $\mathrm{Authorization_{op}(s:S, es:ES, ob:OB)}$ = True.
\end{tabular}}
\iffalse
\multicolumn{6}{l}{-- \ophs is a finite set of operations on Hadoop services.}                                                      \\
\multicolumn{6}{l}{-- UA, OA are finite sets of user and object attribute functions respectively.}                                                      \\
\multicolumn{6}{l}{-- ESA, HSA are finite sets of ecosystem and Hadoop service attribute functions respectively.}                                                      \\
\multicolumn{6}{l}{-- For each attribute att in UA $\cup$ OA $\cup$ ESA $\cup$ HSA, Range(att) is a finite set of atomic values.}   \\
\multicolumn{6}{l}{-- attType: UA = \{set\}, defines user attributes to be set valued only.}                                                      \\
\multicolumn{6}{l}{-- attType: OA $\cup$ ESA $\cup$ HSA = \{set, atomic\}, defines remaining attributes to be set or atomic valued.}                                                      \\
\multicolumn{6}{l}{-- For each attribute $\mathrm{att_u}$ in UA, $\mathrm{att_u}$ : U $\cup$ G $\rightarrow$\; $\mathrm{2^{Range(att_u)}}$ mapping each user or group to a set of attribute values in $\mathrm{Range(att_u)}$.}                                                      \\
%\multicolumn{6}{l}{-- For each attribute $\mathrm{att_{ob}}$ in OA, $\mathrm{att_{ob}}$ : OB $\rightarrow$\; \Big\{ $\mathrm{2^{Range(att_{ob})}}$ mapping each object to a set of attribute values in $\mathrm{Range(att_{ob})}$.} \\
\multicolumn{6}{l}{\begin{tabular}{@{}l@{}}-- Each attribute $\mathrm{att_{ob}}$ in OA maps objects in OB to attribute values. Formally, $\mathrm{att_{ob}}$ : OB $\rightarrow$\; $ \begin{cases} \mathrm{{Range(att_{ob})}} & \text{if attType(att$\mathrm{_{ob}}$) = atomic}\\ \mathrm{2^{Range(att_{ob})}} & \text{if attType(att$\mathrm{_{ob}}$) = set} \\ \end{cases}$ \end{tabular}}\\
\multicolumn{6}{l}{\begin{tabular}{@{}l@{}}-- Each attribute $\mathrm{att_{es}}$ in ESA maps services in ES to attribute values. Formally, $\mathrm{att_{es}}$ : ES $\rightarrow$\; $ \begin{cases} \mathrm{{Range(att_{es})}} & \text{if attType(att$\mathrm{_{es}}$) = atomic}\\ \mathrm{2^{Range(att_{es})}} & \text{if attType(att$\mathrm{_{es}}$) = set} \\ \end{cases}$ \end{tabular}}\\
\multicolumn{6}{l}{\begin{tabular}{@{}l@{}}-- Each attribute $\mathrm{att_{hs}}$ in HSA maps services in HS to attribute values. Formally, $\mathrm{att_{hs}}$ : HS $\rightarrow$\; $ \begin{cases} \mathrm{{Range(att_{hs})}} & \text{if attType(att$\mathrm{_{hs}}$) = atomic}\\ \mathrm{2^{Range(att_{hs})}} & \text{if attType(att$\mathrm{_{hs}}$) = set} \\ \end{cases}$ \end{tabular}}\\

%\multicolumn{6}{l}{-- For each attribute $\mathrm{att_{es}}$ in ESA, $\mathrm{att_{es}}$ : ES $\rightarrow$\; $\mathrm{2^{Range(att_{es})}}$ mapping each ecosystem service to a set of attribute values in $\mathrm{Range(att_{es})}$.} \\
%\multicolumn{6}{l}{-- For each attribute $\mathrm{att_{hs}}$ in HSA, $\mathrm{att_{hs}}$ : HS $\rightarrow$\; $\mathrm{2^{Range(att_{hs})}}$ mapping each Hadoop service to a set of attribute values in $\mathrm{Range(att_{hs})}$.} \\
%\multicolumn{6}{l}{-- For each att in $ \mathrm{ UA \cup OA }$, Range(att) is a finite set of atomic values}                   \\
%\multicolumn{6}{l}{\begin{tabular}[c]{@{}l@{}}-- For each $ \mathrm{att_u }\; \mathrm{in \; UA, \; att_u } : \mathrm{U \cup UG \rightarrow\;2^{Range(att_u)}}$, mapping each user \\ \;\; and user group to a set of values in $\mathrm{Range(att_u)}$\end{tabular}}\\
%\multicolumn{6}{l}{\begin{tabular}[c]{@{}l@{}}-- For each  $ \mathrm{att_o }\; \mathrm{in \; OA, \; att_o} : \mathrm{O \cup OG   \rightarrow  \;2^{Range(att_o)}}$, mapping each object \\ \;\;  and object group to a set of values in $\mathrm{Range(att_o)}$\end{tabular}}                                                                                                         \\
\multicolumn{6}{l}{-- \dirug~ : $ \mathrm{U \rightarrow 2^{G}} $,  mapping each user to a set of groups, equivalently UGA $ \subseteq \Ur \times \Gr $}                                                                                                          \\
%\rowcolor[HTML]{EFEFEF}
%\multicolumn{6}{l}{-- \textsuperscript{**}\dirur~  : $ \mathrm{U \rightarrow 2^{R}} $,  mapping each user to a set of roles, equivalently URA $ \subseteq \Ur \times \R $}\\
%\rowcolor[HTML]{C0C0C0}
%\rowcolor{lightgray!40}
%\multicolumn{6}{l}{-- \dirgr~ : $ \mathrm{G \rightarrow 2^{R}} $,  mapping each group to a set of roles, equivalently GRA $ \subseteq \Gr \times \R $}\\

\multicolumn{6}{l}{-- $\mathrm{GH \subseteq G \times }$G,  a partial order relation  $\succeq_{\textit{g}}$ on G}                                                                                                          \\
%\multicolumn{6}{l}{-- For each attribute $\mathrm{att_{ob}}$ in OA, $\mathrm{att_{ob}}$ : OB $\rightarrow$\; \Big\{ $\mathrm{2^{Range(att_{ob})}}$ mapping each object to a set of attribute values in $\mathrm{Range(att_{ob})}$.} }\\
%\multicolumn{6}{l}{\begin{tabular}[c]{@{}l@{}}-- For each $ \mathrm{att_u }\; \mathrm{in \; UA, \; att_u } : \mathrm{U \cup UG \rightarrow\;2^{Range(att_u)}}$, mapping each user \\ \;\; and user group to a set of values in $\mathrm{Range(att_u)}$\end{tabular}}\\
\iffalse
\multicolumn{6}{l}{-- $\mathrm{\obtag \subseteq OB \times }$Tag, relation between object and object tags}                                                                                                          \\
\multicolumn{6}{l}{-- $\mathrm{\dataprms = 2^{ES \times (OB~ \cup ~Tag)  \times OP}}$,  set of data and service object permissions}                                                                                                          \\
\multicolumn{6}{l}{-- $\mathrm{\hsprms = 2^{HS \times \ophs}}$,  set of Hadoop services permissions}                                                                                                          \\ \fi
\\
%\multicolumn{6}{l}{-- $\mathrm{OGH \subseteq OG \times }$OG, a partial order relation $\succeq_{og} $ on OG}\\
%[\defaultaddspace]
%\hline
%\rowcolor{lightgray}

%[\defaultaddspace]\\
\multicolumn{1}{l}{\textbf{Effective Attributes of Users (Derived Functions)}}                                                                 \\
\multicolumn{6}{l}{\begin{tabular}[c]{@{}l@{}}-- For each attribute $\mathrm{att_u}$ in UA, \\ $ \;\;\;\; \bullet \;\;$ $\mathrm{\effg_{att_{u}}}$ : \Gr~$\rightarrow {2^{\range}}$, defined as $\mathrm{\effg_{att_{u}}(g_i)}$ = $\mathrm{att_u(g_i)}$ $\cup$  $ (\mathrm{\bigcup\limits_{ g \; \in\; \{g_j | g_i \; \succeq_{\textit{g}}\; g_j\} } \effg_{att_{u}}(g))}$. \end{tabular}} \\
\multicolumn{6}{l}{\begin{tabular}[c]{@{}l@{}}-- For each attribute $\mathrm{att_u}$ in UA, \\ $ \;\;\;\; \bullet \;\;$ $\mathrm{\effu_{att_{u}}}$ : \Ur~$\rightarrow {2^{\range}}$, defined as $\mathrm{\effu_{att_{u}}(u)}$ = $\mathrm{att_u(u)}$ $\cup$  $ (\mathrm{\bigcup\limits_{ g \; \in\; \dirug(u)} \effg_{att_{u}}(g))}$. \end{tabular}} \\


%\multicolumn{1}{l}{\textsuperscript{$\dagger\dagger$}\textbf{Role Permission Assignments}}                                                                 \\
%\multicolumn{1}{l}{\cellcolor{lightgray}\textbf{Role Permission Assignments}}                                                                 \\
%\multicolumn{6}{l}{-- $\mathrm{\pahs \subseteq R \times }$\hsprms,  mapping roles to hadoop service permissions. Alternatively, \hsp}                                                                                                          \\
%\multicolumn{6}{l}{\begin{tabular}[c]{@{}l@{}}-- $ \mathrm{\pahs \subseteq R \times }$\hsprms,  mapping roles to Hadoop service permissions. Alternatively, \;\; \hsp~: (r:\R) $\rightarrow  {2^{\hsprms}}$, defined as \\ \hsp(r) = \{p $|$ (r,p) $\in$ \pahs \} \end{tabular}} \\
%\multicolumn{5}{l}{\cellcolor[HTML]{343434}{Maanak}}\\
%\multicolumn{6}{l}{\begin{tabular}[c]{@{}l@{}}-- $\mathrm{\pads \subseteq R \times }$\dataprms,  mapping roles to object permissions. Alternatively, \\\;\; \dsp~: (r:\R) $\rightarrow  {2^{\dataprms}}$, defined as \dsp(r) = \{p $|$ (r,p) $\in$ \pads \} \end{tabular}}
 %\hline
%\multicolumn{6}{l}{-- $\mathrm{\pads \subseteq R \times }$\dataprms,  mapping roles to data service permissions}                                                                                                          \\
%\multicolumn{6}{l}{-- $\mathrm{\pah \subseteq HS \times HS~ \times}$ \ophs,  mapping hadoop service to hadoop service access}\\

\multicolumn{1}{l}{\textbf{Effective Attributes of Subjects}}                                                                                                          \\
\multicolumn{6}{l}{-- \userSub~: \s $\rightarrow \; $U, mapping each subject to its creator user.}                                                                                                          \\
\multicolumn{6}{l}{\begin{tabular}[c]{@{}l@{}}-- For each attribute $\mathrm{att_u}$ in UA, $ \mathrm{\effu_{att_{u}}} : \s \rightarrow \mathrm{2^{Range(att_u)}}$, mapping of subject s to a set of values for its effective \\\;\; attribute $\mathrm{att_{u}}$. It is required that : $ \mathrm{\effu_{att_{u}}}(\mathrm{s}) \subseteq \mathrm{\effu_{att_{u}}}(\userSub(\mathrm{s}))$. \end{tabular}} \\[\defaultaddspace]\\
%\multicolumn{6}{l}{-- $\mathrm{\pah \subseteq HS~ \times}$ \hsprms,  mapping hadoop service to hadoop service access.}\\
%\multicolumn{6}{l}{ \textsuperscript{$\dagger\dagger$}\textbf{Effective Roles of Users (Derived Functions)} }                                                                                                      \\
%\multicolumn{2}{l}{\cellcolor{lightgray}\textbf{Effective Roles of Users (Derived Functions)} }                                                                                                          \\
%\multicolumn{6}{l}{\begin{tabular}[c]{@{}l@{}}$ \;\;\;\; \bullet \;\; \effgr : \Gr \rightarrow {2^{\R}}$, defined as \;\;\;\;\;\; $ \effgr(\mathrm{g_i}) = \dirgr(\mathrm{g_i}) $ $\cup $ $ (\mathrm{\bigcup\limits_{\forall g \; \in\; \{g_j | g_i \; \succeq_{\textit{g}}\; g_j\} } \effgr(g))}$\end{tabular}} \\
%\multicolumn{6}{l}{\begin{tabular}[c]{@{}l@{}}$ \;\;\;\; \bullet \;\; \effur : \Ur \rightarrow {2^{\R}}$, defined as \\ \;\;\;\;\;\; $ \effur(\mathrm{u}) = \dirur(\mathrm{u}) $ $\cup $ $ (\mathrm{\bigcup\limits_{\forall g \; \in\; \dirug(u)} \effgr(g))}$\end{tabular}} \\[\defaultaddspace]\\
%\multicolumn{2}{l}{\cellcolor{lightgray}\textbf{Effective Roles and Permissions of Subjects}}                                                                                                          \\

\multicolumn{1}{l}{\textbf{ Cross Hadoop Services Trust}}                                                                                                          \\
\multicolumn{6}{l}{\begin{tabular}[c]{@{}l@{}}-- trusted-services : \hs~$\rightarrow {2^{\hs}}$ is a required function to map Hadoop services to a set of trusted Hadoop services. \\ \;\; Equivalently, relation service trust written as $\trianglelefteq$ $\subseteq$ $\hs$ $\times$ $\hs$, where $\mathrm{hs_a}$ $\trianglelefteq$ $\mathrm{hs_b}$ iff $\mathrm{hs_b}$ $\in$ trusted-services($\mathrm{hs_a}$), meaning \\\;\; trustee service $\mathrm{hs_b}$ is trusted by trustor service $\mathrm{hs_a}$ and Hadoop service $\mathrm{hs_b}$ can access service $\mathrm{hs_a}$. \;\;\end{tabular}} \\
%\multicolumn{6}{l}{\begin{tabular}[c]{@{}l@{}}-- $\mathrm{\pah \subseteq HS~ \times}$ \hsprms,  mapping Hadoop service to Hadoop service access.\\ \;\; Alternatively, \hshsp~: (hs:\hs) $\rightarrow  {2^{\hsprms}}$, defined as \\\;\; \hshsp(hs) = \{p $|$ (hs,p) $\in$ \pah \} \end{tabular}} \\
\midrule
\multicolumn{2}{l}{ \textbf{Authorization Functions}}                                                                                                          \\
%\multicolumn{2}{l}{-- {Service Authorization Function:}}                                                                                                          \\
\multicolumn{6}{l}{\begin{tabular}[c]{@{}l@{}}-- {Service Authorization Function:} For each op $\in$ \ophs, $\mathrm{Authorization_{op}(s:S, sr:HS \cup ES)}$ is a propositional logic formula \\\;\; returning true or false, which is defined  using the following policy language: \end{tabular}}\\
\multicolumn{6}{l}{\begin{tabular}[c]{@{}l@{}}$\;\;\;\; \bullet \;\; \mathrm{ \alpha \Coloneqq \alpha \land \alpha \;|\; \alpha \vee \alpha \;|\; (\alpha) \;|\; \neg \alpha \;|\; \exists\; x \in set.\alpha  \;|\; \forall\; x \in set.\alpha \;|\;  set \bigtriangleup set \;|\; } $ $ \mathrm{atomic \in set \;|\;  atomic \notin set }$\end{tabular}} \\

\multicolumn{6}{l}{$ \;\;\;\; \bullet \;\; \bigtriangleup \Coloneqq  \; \subset \;|\; \subseteq \;|\; \nsubseteq \;|\; \cap \;|\; \cup $}\\
\multicolumn{6}{l}{$ \;\;\;\; \bullet \;\;\mathrm{  set \Coloneqq {effective}_{att_{u}}(s) \;|\; {att_{sr}}(sr) }$} for $\mathrm{att_{u}}$ $\in $ UA, sr $\in$ ES $\cup$ HS, attType(att) = set\\
\multicolumn{6}{l}{$ \;\;\;\; \bullet \;\; \mathrm{ atomic \Coloneqq {att_{sr}}(sr) \;|\; value }$} sr $\in$ ES $\cup$ HS, attType(att) = atomic\\
\multicolumn{6}{l}{\begin{tabular}[c]{@{}l@{}}-- {Data or Service Objects Authorization Function:} For each op $\in$ OP on objects ob $\in$ OB belonging to ecosystem service es $\in$ ES, \\\;\; $\mathrm{Authorization_{op}(s:S, es:ES, ob:OB)}$ is a propositional logic formula returning true or false, which is defined  using \\\;\; the policy language stated above with following changes \end{tabular}}\\
\multicolumn{6}{l}{$ \;\;\;\; \bullet \;\;\mathrm{  set \Coloneqq {effective}_{att_{u}}(s) \;|\; {att_{es}}(es)\;|\; {att_{ob}}(ob) }$} for $\mathrm{att_{u}}$ $\in $ UA, attType(att) = set\\
\multicolumn{6}{l}{$ \;\;\;\; \bullet \;\; \mathrm{ atomic \Coloneqq {att_{es}}(es) \;|\; att_{ob}(ob) \;|\; value }$} attType(att) = atomic\\
%\multicolumn{6}{l}{\begin{tabular}[c]{@{}l@{}}A subject $\mathrm{s}$ $\in$ S is allowed to perform an operation op $\in$ OP on an object $\mathrm{ob}$  $\in$ OB in ecosystem service es $\in$  ES  if the effective \\ object permissions of subject s include permissions to object ob or to tag t $\in$ Tag associated with object ob. Formally,\\ (es,ob,op) $\in$ \effdp($\mathrm{s)}$ $\lor$\\ ($\exists$ t) [(ob,t) $\in$  \obtag~$\land$ (es,t,op) $\in$ \effdp($\mathrm{s)}$] \end{tabular}}\\
%\multicolumn{6}{l}{ For each operation \userSub~: \s $\rightarrow \; $U, mapping each subject to its creator user}                                                                                                          \\
%\multicolumn{6}{l}{\begin{tabular}[c]{@{}l@{}}$ \;\;\;\; \bullet \;\; \effur : \s \rightarrow {2^{\R}}$, mapping of subject s to a set of roles. It is required that : \\ \;\;\;\;\;\; $ \effur(\mathrm{s}) \subseteq \effur(\userSub(\mathrm{s})) $ \end{tabular}} \\[\defaultaddspace]
%\multicolumn{6}{l}{\begin{tabular}[c]{@{}l@{}}-- For each $\mathrm{att_u }$ in UA, $ \mathrm{effective_{att_u} :S \rightarrow 2^{Range({att_u})}}$, mapping of subject s \\ \;\; to a set of roles. It is required that : \\ \;\; $ \mathrm {effective_{att_u}(s) \subseteq {effective}_{att_u}(SubUser(s))}$\end{tabular}}\\ [\defaultaddspace]
%\multicolumn{6}{l}{\begin{tabular}[c]{@{}l@{}}$ \;\;\;\; \bullet \;\; \effhp : \s \rightarrow {2^{\hsprms}}$, defined as $ \effhp(\mathrm{s}) =  $  $ \mathrm{\bigcup\limits_{\forall r \; \in\; \effur(s)} \hsp(r)}$\end{tabular}} \\[\defaultaddspace]
%\multicolumn{6}{l}{\begin{tabular}[c]{@{}l@{}}$ \;\;\;\; \bullet \;\; \effdp : \s \rightarrow {2^{\dataprms}}$, defined as $ \effdp(\mathrm{s}) =  $  $ \mathrm{\bigcup\limits_{\forall r \; \in\; \effur(s)} \dsp(r)}$\end{tabular}} \\[\defaultaddspace]
\midrule
\multicolumn{6}{l}{\textbf{Access Operation Decision}}\\
\multicolumn{6}{l}{\begin{tabular}[c]{@{}l@{}}-- A subject $\mathrm{s}$ $\in$ S is allowed to perform an operation op $\in$ \ophs on a service sr $\in$  ES $\cup$ HS  if the effective attributes of subject s and \\\;\; attributes of services satisfy policies stated in $\mathrm{Authorization_{op}(s:S, sr:HS \cup ES)}$. \\\;\; Formally, $\mathrm{Authorization_{op}(s:S, sr:HS \cup ES)}$ = True.
\end{tabular}}  \\
\multicolumn{6}{l}{\begin{tabular}[c]{@{}l@{}}-- A subject $\mathrm{s}$ $\in$ S is allowed to perform an operation op $\in$ OP on an object $\mathrm{ob}$  $\in$ OB in ecosystem service es $\in$  ES  if subject is allowed \\\;\; to access services es and the effective  attributes of subject s, the attributes of object ob and service es satisfy policies in \\\;\; $\mathrm{Authorization_{op}(s:S, es:ES, ob:OB)}$.\\\;\; Formally, $\mathrm{Authorization_{access}(s:S, es:ES)}$ = True $\land$ $\mathrm{Authorization_{op}(s:S, es:ES, ob:OB)}$ = True.
\end{tabular}}      \fi               \\
\bottomrule
%\multicolumn{6}{l}{\textsuperscript{**} and \textsuperscript{$\dagger\dagger$} highlight new and modified components respectively with respect to \heac}\\
\end{tabular}}
\end{table*}

